Matryoshka Representation Learning

Learned representations are a central component in modern ML systems, serving a multitude of downstream tasks. When training such representations, it is often the case that computational and statistical constraints for each downstream task are unknown. In this context rigid, fixed capacity representations can be either over or under-accommodating to the task at hand. This leads us to ask: can we design a flexible representation that can adapt to multiple downstream tasks with varying computational resources? Our main contribution is Matryoshka Representation Learning (MRL) which encodes information at different granularities and allows a single embedding to adapt to the computational constraints of downstream tasks. MRL minimally modifies existing representation learning pipelines and imposes no additional cost during inference and deployment. MRL learns coarse-to-fine representations that are at least as accurate and rich as independently trained low-dimensional representations. The flexibility within the learned Matryoshka Representations offer: (a) up to 14x smaller embedding size for ImageNet-1K classification at the same level of accuracy; (b) up to 14x real-world speed-ups for large-scale retrieval on ImageNet-1K and 4K; and (c) up to 2% accuracy improvements for long-tail few-shot classification, all while being as robust as the original representations. Finally, we show that MRL extends seamlessly to web-scale datasets (ImageNet, JFT) across various modalities -- vision (ViT, ResNet), vision + language (ALIGN) and language (BERT). MRL code and pretrained models are open-sourced at https://github.com/RAIVNLab/MRL.

==> TabsNFigs/Cascades.tex <==
\begin{figure}[ht!]
% \vspace{-3mm}
\centering
\resizebox{0.5\columnwidth}{!}{%
\includegraphics[width=0.5\columnwidth]{TabsNFigs/images/CASCADE-vs-MRL.pdf}
}
% \vspace{-3mm}
\caption{\small R50 Cascade accuracy + Few-shot table?}
% }
% \vspace{-5mm}
\label{fig:r50-cascades}
\end{figure}

==> TabsNFigs/Reranking_MainPaper_IN1K_NaivePolicy.tex <==
\begin{table}[h]
\centering
 \caption{Retrieve a shortlist of k-NN with \retdim\space sized representations on \InIk. This shortlist is then reranked with funnel retrieval, which uses a rerank cascade with a one-to-one mapping with a monotonically decreasing shortlist length. This is in an attempt to emulate the performance of retrieval at higher dimensions with substantially lower MFLOPs.}
 \vspace{1mm}
 \resizebox{\columnwidth}{!}{
\begin{tabular}{@{}c|c|c|c|ccccc@{}}
\toprule
\retdim & Rerank Cascade          & Cascade List                            & MFLOPs & Top-1 & Top-5 & Top-10 & mAP@10 & P@10 \\ \midrule
8       & 16$\to$32$\to$64$\to$128$\to$2048   & \multirow{3}{*}{~~200$\to$100$\to$50$\to$25$\to$10} & 10.28  & 70.22 & 82.63 & 85.49  & 64.06  & 68.65   \\
16      & 32$\to$64$\to$128$\to$256$\to$2048  &                                         & 20.54  & 70.90 & 83.96 & 86.85  & 65.19  & 69.97   \\
32      & 64$\to$128$\to$256$\to$512$\to$2048 &                                         & 41.07  & 70.96 & 84.32 & 87.47  & 65.21  & 70.11 \\ \bottomrule 
\end{tabular}
\label{tab:rerankcascade_in1k_condensed}
}
\end{table}

==> TabsNFigs/inat.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\centering
\caption{Few-shot accuracy on ImageNetV2 for 1000 way classification. \MH~performs equally to \FF~across all shot and representation sizes. We also observe that accuracy saturates at a lower representation size for lower shot numbers. For example, at 1-shot a rep. size of 32 performs equally to 2048.}
\vspace{1mm}
\begin{tabular}{@{}
c |
c |
c
c 
c 
c 
c @{}}
\toprule
$d$& Method &
  1-Shot &
  3-Shot &
  5-Shot &
  7-Shot &
  9-Shot \\ \midrule
  \multirow{2}{*}{\begin{sideways}8\end{sideways}}
& FF & 35.41     & 45.73     & 49.23     & 50.89     & 51.72     \\
& MH & 35.37     & 45.69     & 49.25     & 50.85     & 51.73     \\ \midrule
\multirow{2}{*}{\begin{sideways}16\end{sideways}}
& FF & 40.88     & 53.96     & 57.36     & 58.72     & 59.39     \\
& MH & 40.90     & 53.94     & 57.37     & 58.65     & 59.29     \\ \midrule
\multirow{2}{*}{\begin{sideways}32\end{sideways}}
& FF & 41.41     & 54.88     & 58.28     & 59.63     & 60.40     \\
& MH & 41.40     & 54.91     & 58.30     & 59.65     & 60.45     \\ \midrule
\multirow{2}{*}{\begin{sideways}64\end{sideways}}
& FF & 41.25     & 54.83     & 58.29     & 59.82     & 60.61     \\
& MH & 41.28     & 54.80     & 58.32     & 59.77     & 60.69 \\ \midrule
\multirow{2}{*}{\begin{sideways}128\end{sideways}}
& FF & 41.36     & 54.90     & 58.50     & 60.05     & 60.90     \\
& MH & 41.38     & 54.95     & 58.50     & 60.06     & 60.83     \\ \midrule
\multirow{2}{*}{\begin{sideways}256\end{sideways}}
& FF & 41.36 & 54.90 & 58.50 & 60.05 & 60.90 \\
& MH & 41.38 & 54.95 & 58.50 & 60.06 & 60.83 \\ \midrule
\multirow{2}{*}{\begin{sideways}512\end{sideways}}
& FF & 41.36 & 55.05 & 58.70 & 60.19 & 61.02 \\
& MH & 41.34 & 55.14 & 58.78 & 60.40 & 61.18 \\ \midrule
\multirow{2}{*}{\begin{sideways}1024\end{sideways}} & FF & 41.32 & 55.20 & 58.85 & 60.46 & 61.38 \\
& MH & 41.31 & 55.24 & 58.86 & 60.42 & 61.34 \\ \midrule
\multirow{2}{*}{\begin{sideways}2048\end{sideways}} & FF & 41.18 & 55.09 & 58.77 & 60.38 & 61.34 \\
& MH & 41.16 & 55.10 & 58.77 & 60.40 & 61.28 \\
\bottomrule
\end{tabular}
\label{Tab:inat}
\end{table}

==> TabsNFigs/superclass.tex <==
\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.8\columnwidth]{TabsNFigs/images/superclass_acc.pdf}
    \caption{Improvement of within-superclass classification with increasing representation size for several selected supervlasses. We observe that superclasses such as ``oscine (songbird)'' have a clear distinction between the object and background and thus predictions using representation size of 8 also lead to a good performance.}
    \label{fig:superclass}
\end{figure}

==> TabsNFigs/superclass_barplot.tex <==
% \setlength{\textfloatsep}{5pt}
% \begin{wrapfigure}{r}{0.6\columnwidth}\vspace{-4mm}
%  \centering
%  \vspace{-2pt}
%  \includegraphics[width=0.57\columnwidth,]{TabsNFigs/images/superclass.pdf}
%  \vspace{-2pt}
%  \caption{Improvement of 31-way superclass classification with increasing representation size for MRL and FF models.}
% \label{fig:superclass_barplot_main}	
% \vspace{-6pt}
% \end{wrapfigure}
